10 Years Later: The Mathematics Subject Classification and Linked Open Data

Ten years ago, the Mathematics Subject Classification MSC 2010 was released, and a corresponding machine-readable Linked Open Data collection was published using the Simple Knowledge Organization System (SKOS). Now, the new MSC 2020 is out. This paper recaps the last ten years of working on machine-readable MSC data and presents the new machine-readable MSC 2020. We describe the processing required to convert the version of record, as agreed by the editors of zbMATH and Mathematical Reviews, into the Linked Open Data form we call MSC2020-SKOS. The new form includes explicit marking of the changes from 2010 to 2020, some translations of English code descriptions into Chinese, Italian, and Russian, and extra material relating MSC to other mathematics classification efforts. We also outline future potential uses for MSC2020-SKOS in semantic indexing and sketch its embedding in a larger vision of scientific research data.

==> 06_llncs_acknowledgements.tex <==
%\noindent\textbf{Acknowledgments} Our research was supported by the German Research Foundation (DFG grant GI 1259/1).


==> 07_reference.tex <==
%TODO once your paper was published, update the reference below for the bib-entry in the preprints

%TODO Update the following line whenever you change the key of the bibtex entry (currently LastnameYYYY) above.
\newcommand{\theReferenceText}{\fullcite{LastnameYYYY}}

